3DEgo: 3D Editing on the Go!

We introduce 3DEgo to address a novel problem of directly synthesizing photorealistic 3D scenes from monocular videos guided by textual prompts. Conventional methods construct a text-conditioned 3D scene through a three-stage process, involving pose estimation using Structure-from-Motion (SfM) libraries like COLMAP, initializing the 3D model with unedited images, and iteratively updating the dataset with edited images to achieve a 3D scene with text fidelity. Our framework streamlines the conventional multi-stage 3D editing process into a single-stage workflow by overcoming the reliance on COLMAP and eliminating the cost of model initialization. We apply a diffusion model to edit video frames prior to 3D scene creation by incorporating our designed noise blender module for enhancing multi-view editing consistency, a step that does not require additional training or fine-tuning of T2I diffusion models. 3DEgo utilizes 3D Gaussian Splatting to create 3D scenes from the multi-view consistent edited frames, capitalizing on the inherent temporal continuity and explicit point cloud data. 3DEgo demonstrates remarkable editing precision, speed, and adaptability across a variety of video sources, as validated by extensive evaluations on six datasets, including our own prepared GS25 dataset. Project Page: https://3dego.github.io/

==> sec/backup/evaluation.tex <==
% \begin{table}[tb]
% \centering
% \caption{\footnotesize Quantitative evaluation of 200 edits across 50 scenes of Gauss50 dataset assessing text alignment and frame consistency in CLIP space for 3D scene editing. 
%  }
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc}
% \hline
%  & \multicolumn{3}{c|}{\textbf{GS50}} & \multicolumn{3}{c}{\textbf{CO3D-v2}} \\
% \textbf{Method} & \textbf{DreamEditor} & \textbf{IN2N~\cite{Instruct-NeRF2NeRF}} & \textbf{Ours} & \textbf{IN2N~\cite{Instruct-NeRF2NeRF}}  & \textbf{IN2N~\cite{Instruct-NeRF2NeRF}} & \textbf{IN2N~\cite{Instruct-NeRF2NeRF}}\\ \hline
% \textbf{CTIS$\uparrow$} & 0.2801 & 0.2788 & 0.2801 & 0.2788 \\
% \textbf{CDCR$\uparrow$} & 0.9881 & 0.9850 & 0.9881 & 0.9850 \\
% \textbf{E-PSNR$\uparrow$} & 26.47 & 25.34 & 26.47 & 25.34 \\ \hline
% \end{tabular}
% }
% \label{tab:merged_table}
% \end{table}

\begin{table}[ht]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt} % Slightly reduce space between columns
\renewcommand{\arraystretch}{1.2} % Adjust vertical spacing
\caption{\footnotesize Quantitative evaluation of 200 edits across 50 scenes of Gauss50 dataset assessing text alignment and frame consistency in CLIP space for 3D scene editing. 
 }
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccccccc}
\hline
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Datasets\end{tabular}} & & \multicolumn{3}{c}{DreamEditor} && \multicolumn{3}{c}{IN2N} && \multicolumn{3}{c}{Ours} \\ 
\cline{4-6} \cline{8-10} \cline{12-14} 
& & & CTIS$\uparrow$ & CDCR$\uparrow$ & E-PSNR$\uparrow$ && CTIS$\uparrow$ & CDCR$\uparrow$ & E-PSNR$\uparrow$ && CTIS$\uparrow$ & CDCR$\uparrow$ & E-PSNR$\uparrow$ \\ 
\hline
% Your table content here
\hline
\end{tabular}
}
\label{tab:comparison}
\end{table}




% \begin{table}[tb]
% \centering
% \caption{\footnotesize Quantitative evaluation of scene edits in terms of text alignment and frame consistency in CLIP space where our approach demonstrates the highest consistency in comparison to other Pose-free methods}
% \resizebox{0.96\textwidth}{!}{
% \begin{tabular}{lccc}
% \hline
% \textbf{Method} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}CLIP Text-Image\\
% Direction Similarity$\uparrow$\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}CLIP Direction\\
%  Consistency$\uparrow$\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Edit\\ PSNR$\uparrow$\end{tabular}} \\ \hline
% \textbf{NeRF-Art}~\cite{wang2023nerf} & 0.2755 & 0.9672 & 22.15 \\
% \textbf{Control4D~\cite{shao2023control4d}} & 0.2503 & 0.9751 & 20.89 \\
% \textbf{DreamEditor~\cite{zhuang2023dreameditor}} & 0.2604 & 0.9802 & 21.76 \\
% \textbf{IN2N}~\cite{Instruct-NeRF2NeRF} & 0.2788 & 0.9850 & 25.34 \\
% \textbf{Ours}             & \textbf{0.2801} & \textbf{0.9881} & \textbf{26.47} \\ \hline
% \end{tabular}
% }

% \label{tab:tab2}

% \end{table}

% \begin{table}[tb]
% \centering
% \caption{\footnotesize Quantitative evaluation of 3D edited scene edits in terms of text alignment and frame consistency in CLIP space. Methods listed here use poses initialized with SfM and first train the 3D model on original images before editing the scene condition on the textual prompt. }
% \resizebox{0.96\textwidth}{!}{
% \begin{tabular}{lccc}
% \hline
% \textbf{Method} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}CLIP Text-Image\\
% Direction Similarity$\uparrow$\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}CLIP Direction\\
%  Consistency$\uparrow$\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Edit\\ PSNR$\uparrow$\end{tabular}} \\ \hline
% \textbf{NeRF-Art}~\cite{wang2023nerf} & 0.2755 & 0.9672 & 22.15 \\
% \textbf{Control4D~\cite{shao2023control4d}} & 0.2503 & 0.9751 & 20.89 \\
% \textbf{DreamEditor~\cite{zhuang2023dreameditor}} & 0.2604 & 0.9802 & 21.76 \\
% \textbf{IN2N}~\cite{Instruct-NeRF2NeRF} & 0.2788 & 0.9850 & 25.34 \\
% \textbf{Ours}             & \textbf{0.2801} & \textbf{0.9881} & \textbf{26.47} \\ \hline
% \end{tabular}
% }

% \label{tab:tab3}

% \end{table}
\section{Evaluation}
\subsection{Implementation Details}
In our approach, we employ PyTorch~\cite{paszke2019pytorch} for the development, specifically focusing on 3D Gaussian splatting. GPT-3.5 Turbo~\cite{brown2020language} is used for identifying the editing attributes to identify the KEA. For segmentation purposes, SAM~\cite{kirillov2023segment} is used to generate the masks based on the key editing attributes identifying the KIA. For zero-shot point tracking, we employ a point-tracker as proposed in~\cite{rajivc2023segment}. The editing tasks are facilitated by the Instruct Pix2Pix~\cite{brooks2022instructpix2pix} 2D diffusion model by incorporating the masks to limit the editing within KEA. For point-cloud initialization, we use a pre-trained depth estimator proposed by~\cite{yang2024depth}. 

\subsection{Baseline and Datasets.}
We carry out experiments across a variety of public datasets as well as our proprietary \textbf{GS50} dataset (to be released publicly), which we prepared in-house.
\noindent\textbf{GS25 Dataset.}
 It comprises 25 casually captured monocular videos using mobile phones for comprehensive 3D scene analysis.  This approach ensures the dataset's utility in exploring and enhancing 360-degree real-world scene reconstruction technologies. 


\noindent\textbf{Public Datasets.} To further assess the efficacy of the proposed 3D editing framework, we also conducted comparisons across four public datasets: (i) IN2N \cite{haque2023instruct}, (ii) Mip-NeRF~\cite{barron2022mipnerf360},(iii) NeRFstudio Dataset \cite{tancik2023nerfstudio}, and (iv) CO3D-V2~\cite{reizenstein2021common}.  We specifically validate the robustness of our approach on the CO3D dataset, which comprises thousands of object-centric videos. These videos feature complex and challenging camera movements, with each video capturing a complete object within the frame as the camera performs a full circular motion around it.

In our study, we introduce a unique problem, making direct comparisons with prior research challenging. Nonetheless, to assess the robustness of our method, we contrast it with state-of-the-art (SOTA) 3D editing techniques that rely on poses derived from COLMAP. Additionally, we present quantitative evaluations alongside pose-free 3D reconstruction approaches, specifically NoPeNeRF~\cite{bian2023nope}, and BARF~\cite{lin2021barf}. In the pose-free comparison, we substitute only our 3D scene reconstruction component with theirs while maintaining our original editing framework unchanged.
we primarily present the qualitative comparisons with IN2N \cite{haque2023instruct} due to space constraint, the benchmark for text-driven NeRF editing that requires a pre-trained 3D model and SfM poses.

\begin{figure}[t!]
\vspace{-5mm}
\centering
    \includegraphics[width=1\linewidth, trim={0cm 1.5cm 0cm 0cm}, clip]{figures/figure6.pdf}
\vspace{-2mm}
\caption{\footnotesize \textbf{Comparison with IN2N}}
\label{fig:comparison}
\end{figure}

\subsection{Qualitative Evaluation}
Our framework enables us to perform ambitious edits such as full-body transformations and facial swaps with high realism and control. Also, our method adapts to changes in geometry and appearance, allowing for a broader range of creative and realistic scene modifications.

\noindent\textbf{Local Editing.}
Our method demonstrates exceptional prowess in local editing, enabling precise modifications within specific regions of a 3D scene without affecting the overall integrity. This capability is showcased through targeted edits, such as altering the color of specific facial areas, ensuring that modifications are both subtle and impactful. Such precision in local editing allows for detailed customization according to user instructions, exemplifying our method's ability to achieve nuanced adjustments that adhere closely to the desired outcomes.

\noindent\textbf{Geometric Editing.}
In geometric editing, our approach exhibits a strong ability to modify the shape and structure of objects within a 3D scene. This is particularly evident in our manipulation of human subjects and open 3D environments, where we implement geometric alterations alongside texture modifications. Our technique adeptly handles complex transformations, maintaining 3D consistency across edits. This not only includes simple shape changes but also extends to more complex geometric manipulations, showcasing our method's flexibility and control in reshaping the 3D world.
% \begin

\begin{figure}[t!]
\vspace{-5mm}
\centering
    \includegraphics[width=1\linewidth, trim={0cm 0cm 0cm 0cm}, clip]{figures/multi-bull.pdf}
\vspace{-2mm}
\caption{\footnotesize \textbf{Figure4: kkkkkkkkkkk}}
\label{fig:comparison}
\end{figure}

\noindent\textbf{3D Object Removal}
The goal of 3D object elimination is to entirely remove an object from a 3D environment, potentially leaving behind voids due to the lack of observational data. For the object removal task, we identify and remove the regions based on the 2D mask, $M$. Subsequently, we focus on inpainting these "invisible regions" in the original 2D frames using LAMA ~\cite{suvorov2022resolution}. In Figure~\ref{fig:removal}, we demonstrate our DirectEdit3D's effectiveness in object removal compared to Gaussian Grouping~\cite{ye2023gaussian}. As illustrated in Figure~\ref{fig:removal}, our method's reconstruction output notably surpasses that of Gaussian Grouping~\cite{ye2023gaussian} in terms of retaining spatial accuracy and ensuring consistency across multiple views. Particularly in complex scenarios involving large objects, our approach successfully distinguishes between the object and its surrounding environment. 

\noindent\textbf{Multi-Attribute Editing.}
Our method excels in multi-attribute editing, seamlessly combining changes across color, texture, and geometry within a single coherent edit. This multifaceted approach is demonstrated in complex scenes with multiple objects, where we successfully apply distinct edits to background and foreground elements, including occluded objects. Through strategic multi-attribute editing, we ensure that each modification contributes to a harmonious overall scene, highlighting our method's capability to orchestrate comprehensive scene transformations.

Comparing our method to Instruct-NeRF to NeRF (IN2N), it becomes clear that our approach offers superior performance in distinguishing and editing specific objects within the foreground, preserving the background's integrity. 
\subsection{Quantitative Evaluation}
\noindent\textbf{Evaluation Criteria.} In our quantitative analysis, we employ three key metrics: \textit{CLIP Text-Image Direction Similarity(CTIS)}~\cite{gal2021stylegan}, \textit{CLIP Direction Consistency Score (CDCR)}~\cite{Instruct-NeRF2NeRF}, and \textit{Edit PSNR(EPSNR)}. The CLIP Directional Score measures how well changes in text descriptions align with visual modifications in the images. Meanwhile, the CLIP Consistency Score evaluates the cosine similarity of CLIP embeddings for successive frames along a new camera path. The Edit PSNR metric assesses both the cosine similarity and PSNR (Peak Signal-to-Noise Ratio) across all rendered views, comparing the edited NeRF to the original NeRF. Through this comparison, it's evident that our approach ensures higher fidelity and consistency in the scene edits relative to the original scene.

\noindent\textbf{Evaluation Through User Feedback.}
To assess the subjective aspects of scene editing effectiveness, we organized a user study that pits our approach against leading state-of-the-art (SOTA) methods. This study collected 100 votes, focusing on crucial aspects such as 3D consistency, fidelity to the original scene, and compliance with textual instructions. Results, illustrated in Figure~\ref{fig:user_study}, show a clear preference for our method across these categories. Details of the user study are in the \textit{\textcolor{blue}{supplementary materials}.}


\section{Ablation Study and Analysis}



==> sec/backup/intro.tex <==
\section{Introduction}
\label{sec:intro}
\begin{wrapfigure}{r}{0.5\textwidth} % Position on the right and half of the text width
 % Adjust the spacing as needed
 \vspace{-7mm}
    \centering
    \includegraphics[width=0.48\textwidth, trim={6cm 1.5cm 6cm 2cm}, clip]{figures/figure1.pdf} % Adjust the width slightly less than wrapfigure width for padding
\caption{\footnotesize { Existing T2I editing frameworks such as~\cite{brooks2022instructpix2pix}, encounter notable challenges in maintaining consistency across multiple views. }}
\label{fig:fig1}
\vspace{-4mm}
 % Adjust the spacing as needed
\end{wrapfigure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{eccv3_2.png}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}



In the pursuit of constructing photo-realistic 3D scenes from monocular video sources, it is a common practice to use Structure-from-Motion (SfM) library, COLMAP~\cite{schonberger2016structure} for camera pose estimation\cite{schonberger2016structure}. This step is critical for aligning frames extracted from the video, thereby facilitating the subsequent process of 3D scene reconstruction. To further edit these constructed 3D scenes, a meticulous process of frame-by-frame editing based on textual prompts is often employed. Recent works, such as IN2N~\cite{haque2023instruct}, estimate poses from frames using  SfM to initially train an unedited 3D scene.  Upon initializing a 3D model, the training dataset is iteratively updated by adding edited images at a consistent rate of editing.   This process of iterative dataset update demands significant computational resources and time. Due to challenges with initial edit consistency, IN2N training necessitates the continuous addition of edited images to the dataset over a significantly large number of iterations. This issue stems from the inherent limitations present in Text-to-Image (T2I) diffusion models, where achieving prompt-consistent edits across multiple images—especially those capturing the same scene—proves to be a formidable task. As illustrated in Fig.~\ref{fig:fig1}, employing the same target prompt can lead to varying outcomes across different views within the scene, highlighting the issue of inconsistent edits or styles. 
Such inconsistencies significantly undermine the effectiveness of 3D scene modifications, particularly when these altered frames are leveraged to generate unique views. 
\begin{wrapfigure}{r}{0.5\textwidth} % Position on the right and half of the text width
 % Adjust the spacing as needed
    \centering
    \vspace{-5.5mm}
    \includegraphics[width=0.48\textwidth, trim={4cm 2.5cm 4cm 3cm}, clip]{figures/figure2.pdf} % Adjust the width slightly less than wrapfigure width for padding
\caption{\footnotesize{ Our method, \textbf{DirectEdit3D} achieves precise editing without using any SfM poses. Here, we constructed original \textbf{3DGS}~\cite{kerbl20233d}, \textbf{ IN2N}~\cite{haque2023instruct}, and \textbf{IP2P+COLMAP} using COLMAP~\cite{colmap} poses. To construct the IP2P+COLMAP 3D scene, we train nerfacto~\cite{tancik2023nerfstudio} model on IP2P~\cite{brooks2022instructpix2pix} edited frames without iterative dataset update.}}
\label{fig:fig2}
\vspace{-4mm}
 % Adjust the spacing as needed
\end{wrapfigure}


% \begin{figure}[t!]
% \vspace{-5mm}
% \centering
%     \includegraphics[width=1\linewidth, trim={1cm 1.5cm 1cm 1cm}, clip]{figures/figure1.pdf}
% \vspace{-2mm}
% \caption{\footnotesize \textbf{Multi-View Inconsistency in Current Text-to-Image (T2I)
% Editing Models: The current T2I editing model [6] faces significant challenges with multi-view consistency. This issue adversely affects the quality of 3D scene editing, especially when these edited views are used to
% synthesize novel views. This specific limitation is also acknowledged in
% InstructN2N [18]. It is important to note that this inconsistency is particularly problematic when rendering is performed without re-training, which
% aligns with the objectives of our study.}}
% \label{fig:intro}
% \end{figure}

In this work, we address a novel problem of efficiently reconstructing 3D scenes directly from monocular videos aligned with the editing textual prompt. Specifically, We apply a diffusion model~\cite{brooks2022instructpix2pix} to edit every frame of a given monocular video before creating a 3D scene. Given that the edited frames from IP2P~\cite{brooks2022instructpix2pix} lack consistency across different views, we acknowledge that initializing COLMAP poses with the original frames is not required (see Figure~\ref{fig:fig2}). Also, the pose estimation step is time-consuming and prone to failure, especially in scenes with textureless surfaces or repetitive patterns due to its reliance on feature extraction. Therefore, our framework directly creates an edited 3D scene from a given monocular video without the traditional reliance on COLMAP for camera pose estimation and without initializing an original (unedited) 3D scene. Hence, our method \textbf{DirectEdit3D} condenses a three-stage 3D editing process into a single-stage, unified and efficient framework as shown in Figure~\ref{fig:fig3}.

Our framework fundamentally utilizes the Gaussian Splatting (GS) technique, capitalizing on the temporal continuity of video data and the explicit representation of point clouds. Unlike recent approaches that attempt to minimize the dependency on Structure-from-Motion (SfM) by embedding pose estimation within the Neural Radiance Fields (NeRFs~\cite{mildenhall2021nerf}) framework~\cite{wang2021nerfmm, lin2021barf, bian2023nope}, our method acknowledges the inherent challenges posed by NeRF's implicit scene representation. Specifically, the implicit nature of NeRF complicates the simultaneous tasks of 3D scene reconstruction and camera registration due to additional optimization constraints. The introduction of 3D Gaussian Splatting~\cite{kerbl20233d} has broadened the capabilities of volumetric rendering beyond NeRFs, enabling the use of point clouds. Originally designed to work with pre-computed camera poses, 3D Gaussian Splatting presents us with the possibility to synthesize views and construct edited 3D scenes from monocular videos without the need for SfM pre-processing, thus overcoming one of NeRF's significant limitations.


Our method grows the 3D Gaussians of the scene continuously, from the edited frames, as the camera moves, eliminating the need for pre-computed camera poses and 3D model initialization on original un-edited frames; therefore, directly accommodating the edited frames' inconsistencies.

Our contributions are as follows:
\begin{itemize}
    \item A novel framework for direct monocular video to 3D scene reconstruction that integrates IP2P editing diffusion models for frame editing based on textual prompts, without the need for COLMAP poses.
    \item The introduction of a COLMAP-free approach using 3D Gaussian splatting for 3D scene reconstruction, facilitating efficient and flexible editing and reconstruction processes.
    \item Extensive evaluation on the Tanks and Temples dataset~\cite{Knapitsch2017} and CO3D dataset~\cite{reizenstein2021common}, demonstrating superior performance in view synthesis and competitive accuracy in camera pose estimation compared to existing methods as shown in Figure~\cite{fig:fig4}.
\end{itemize}



% Our method not only provides a robust solution to the challenges of photo-realistic scene reconstruction and view synthesis but also opens new avenues for integrating machine learning techniques with traditional computer vision frameworks, paving the way for more efficient and flexible 3D scene modeling.



\begin{figure}[t!]
\vspace{-5mm}
\centering
    \includegraphics[width=1\linewidth, trim={2cm 1cm 2cm 1cm}, clip]{figures/teaser.pdf}
\vspace{-2mm}
\caption{\footnotesize \textbf{Teaser}}
\label{fig:fig5}
\end{figure}


==> sec/backup/method.tex <==

\section{Method}
\label{sec:method}
Given a sequence of unposed images alongside camera intrinsics, we aim to recover the camera poses in sync with the edited frames and reconstruct a photo-realistic 3D scene conditioned on the textual prompt. To achieve this, we propose \textbf{T}extual \textbf{P}rompts as catalysts for \textbf{P}ose-\textbf{F}ree \textbf{3D} Scene Generation from Monocular Video Footage (DirectEdit3D) an innovative approach that leverages the power of 3D Gaussian Splatting (3DGS~\cite{kerbl20233d}) and simultaneous camera pose optimization. 

\subsection{Preliminaries:}
% \noindent\textbf{3D Gaussian Splatting}
\label{sec:gau_splat}
In the domain of 3D scene modeling, 3D Gaussian splatting~\cite{kerbl20233d} emerges as a notable method. The method's strength lies in its succinct Gaussian representation coupled with an effective differential rendering technique, facilitating real-time, high-fidelity visualization. This approach models a 3D environment using a collection of point-based 3D Gaussians, denoted as $\mathcal{H} = \{h_1, h_2, ..., h_G\}$, where each $h_g = \{\mu_g, \Sigma_g, c_g, \alpha_g\}$ for $g$ ranging from 1 to $G$. Here, $\mu \in \mathbb{R}^3$ specifies the Gaussian's center location, $\Sigma\in \mathbb{R}^{3 \times 3}$ is the covariance matrix capturing the Gaussian's shape, $c \in \mathbb{R}^3$ is the color vector in RGB format represented in
the three degrees of spherical harmonics (SH) coefficients, and $\alpha \in \mathbb{R}$ denotes the Gaussian's opacity level.
To optimize the parameters of 3D Gaussians to represent the scene, we need to render them into images in a differentiable manner. The rendering is achieved by approximating the projection of a 3D Gaussian along the depth dimension into pixel coordinates expressed as:
\begin{equation}
    C = \sum_{i \in \mathcal{P}} c_i \tau_i \prod_{k=1}^{i-1} (1 - \alpha_k),
    \label{eq:1}
\end{equation}
where $\mathcal{P}$ are ordered points overlapping the pixel, and $\tau_i = \alpha_i e^{-\frac{1}{2}(x_i)^T\Sigma^{-1}(x_i)}$ quantifies the Gaussian's contribution to a specific image pixel, with $x_i$ measuring the distance from the pixel to the center of the $i$-th Gaussian. 
In the original 3DGS~\cite{kerbl20233d}, initial Gaussian parameters are refined to fit the scene, guided by ground truth poses obtained using SfM. Through differential rendering, the Gaussians' parameters, including position $\mu$, shape $\Sigma$, color $c$, and opacity $\alpha$, are adjusted using a photometric loss function. In our work, we eliminate the SfM pose estimation step, a process that will be elaborated upon in subsequent sections.
\subsection{2D Editing with Key Editing Areas:}
\begin{wrapfigure}{r}{0.5\textwidth} % Position on the right and half of the text width
 % Adjust the spacing as needed
    \centering
    \vspace{-5.5mm}
    \includegraphics[width=0.48\textwidth, trim={4cm 2.5cm 4cm 3cm}, clip]{figures/figure2.pdf} % Adjust the width slightly less than wrapfigure width for padding
\caption{\footnotesize{Extracting 2D Masks}}
\label{fig:fig6}
\vspace{-4mm}
 % Adjust the spacing as needed
\end{wrapfigure}
In the first step, we perform 2D editing with key editing areas (KEA) based on the user-provided video, $V$, and editing prompt, $\mathcal{T}$. 
The process begins with extracting frames $\{f_1, f_2, \ldots, f_n\}$ from the video $V$, where each $f_i$ represents an individual frame, $V \rightarrow \{f_1, f_2, \ldots, f_n\}$. Then, the user's textual prompt $\mathcal{T}$ undergoes analysis via a Large Language Model $\mathcal{L}$ to extract multiple key editing attributes, $\{A_1, A_2, \ldots, A_k\}$, where each $A_j$ is a distinct attribute identified for editing, $   \mathcal{L} (\mathcal {T}) \rightarrow \{A_1, A_2, \ldots, A_k\}.$ 

% \noindent \textbf{Multi-View Consistent Mask Generation.}
With the identified key attributes, the segmentation model, $\mathcal{S}$ processes each frame $f_i$ to generate a mask $M_i$ for the regions designated for editing, based on $\{A_1, A_2, \ldots, A_k\}$ such that pixels in $M_i$ corresponding to KEA are 1 and rest are 0. 
\begin{equation}
    \mathcal{S}(f_i, \{A_1, A_2, \ldots, A_k\}) \rightarrow M_i, \quad \forall i \in \{1, \ldots, n\}
\end{equation}
A 2D diffusion model $\mathcal{E}$ then edits only the masked regions of each frame $f_i$, using the masks $M_i$, resulting in a series of edited frames $\{E_1, E_2, \ldots, E_n\}$the original images, $f_i$, guided by the user's instructions $\mathcal{T}$. 
\begin{equation}
    \mathcal{E}(f_i, M_i) \rightarrow E_i, \quad \forall i \in \{1, \ldots, n\}
\end{equation}
As discussed above, differing from IN2N \cite{haque2023instruct} that incorporates edited images gradually over several training iterations, our approach involves editing the entire dataset at once before the training starts. Therefore, to obtain multiple edited views that are consistent with one another, we must ensure multi-view consistent mask generation. As 
$\mathcal{S}$ doesn't guarantee consistent masks across the views of a casually recorded monocular video,  we utilize a zero-shot point tracker~\cite{rajivc2023segment} to ensure uniform mask generation across the views. The procedure starts by identifying query points in the initial video frame using the ground truth mask. Query points are extracted from these ground truth masks employing the K-Medoids~\cite{park2009simple} sampling method. This method utilizes the cluster centers from K-Medoids clustering as query points. This approach guarantees comprehensive coverage of the object's various sections and enhances resilience to noise and outliers.
% \subsubsection{Multi-view Consistent 2D Editing.}

\begin{figure}[t!]
\vspace{-5mm}
\centering
    \includegraphics[width=1\linewidth, trim={1cm 3cm 1cm 3cm}, clip]{figures/figure3.pdf}
\vspace{-2mm}
\caption{\footnotesize \textbf{Method}}
\label{fig:fig5}
\end{figure}
 
 


\subsection{Decoupled 3D Scene Reconstruction}
After multi-view consistent 2D editing is achieved across all frames of the given video, $V$, we leverage the edited frames $E_i$ and their corresponding masks $M_i$ to construct a 3D scene without any SfM pose initialization. Due to the explicit nature of 3DGS~\cite{kerbl20233d},  determining the camera poses is essentially equivalent to estimating the transformation of a collection of 3D Gaussian points. However, SE(3) transformation parametrization for estimating poses requires decoupled scene optimization for KEA and non-KEA Gaussians. Leveraging the explicit nature of 3DGS~\cite{kerbl20233d}, we assign a KEA identity to each Gaussian, enabling decoupled learning of transformation parameters. The process of assigning these identities and their impact on pose estimation during 3D scene reconstruction training will be discussed next.


\subsubsection{3D Gaussians Parameterization for Precise Editing.}
\label{sec:gaussian_parameter}
Projecting the KEA from the image space into 3D Gaussians, $h$, utilizing $M_i$ to assign a KEA identity is crucial for precise editing and accurate pose estimation.  Specifically, we introduce a vector, $m$ associated with the Gaussian point, $h = \{\mu, \Sigma, c, \alpha, m\}$ in the 3D Gaussian set, $\mathcal{H}_i$ of the $i_{th}$ frame. The parameter  $m$ is a learnable vector of length 2 corresponding to the number of labels in the segmentation map, $M$. We optimize the newly introduced parameter $m$  to represent KEA identity during training. However, unlike the view-dependent Gaussian parameters, the KEA Identity remains uniform across different rendering views. Gaussian KEA identity ensures the continuous monitoring of each Gaussian's categorization as they evolve, thereby enabling the selective application of gradients, and the exclusive rendering of targeted objects, markedly enhancing processing efficiency in intricate scenes. In our context, the use of selective gradients is crucial because we propose to have a decoupled scene reconstruction. If this is not carefully managed, even minor inconsistencies in the frames edited initially can result in a challenging "chicken and egg" problem.

% initially set to 0, indicating that it is outside the Gaussian KEA, and a value of 1 signifies its inclusion within the KEA. 
% This addition of the KEA score as a parameter makes it easier to dynamically adjust new points during the densification process.
% The newly added points inherit the KEA identity of their progenitors, ensuring the perpetuation of an accurate 3D semantic mask throughout the training duration. 



% because the learnable affine transformation matrix, $\mathcal{M}$, is designed to specifically address Gaussians with a KEA score of 0. 

% \noindent\textbf{Transformation Parametrization for Pose Estimation}
Next, we delve into the training pipeline in detail and will discuss the role of KEA identity during the proposed training mechanism which consists of two stages: \textit{(i)} Relative Pose Estimation with Single View Addition, and \textit{(ii)} Global 3D Scene Expansion. 

\noindent \textbf{Single View Initialization.} To begin the training process, , we randomly pick a specific frame, denoted as \(E_i\). We then employ a pre-trained monocular depth estimator, symbolized by \(\mathcal{D}\), to derive the depth map \(D_i\) for \(E_i\). Utilizing $D_i$, which provides strong geometric cues independent of camera parameters, we initialize 3DGS with points extracted from monocular depth through camera intrinsics and orthogonal projection. This initialization step involves learning a set of 3D Gaussians $\mathcal{H}_i$ to minimize the photometric discrepancy between the rendered and current frames $E_i$. The photometric loss, $\mathcal{L}_{rgb}$,  optimize the conventional 3D Gaussian parameters including color $c$, covariance $\Sigma$, mean $\mu$, and opacity $\alpha$. However, to initiate the KEA identity and adjust \(m_g\) for 3D Gaussians, merely relying on \(\mathcal{L}_{rgb}\) proves insufficient. Hence, we propose the KEA loss, denoted as \(\mathcal{L}_{KEA}\), which encompasses the 2D mask \(M_i\) corresponding to $E_i$. Overall, 3D Gaussian optimization is defined as,
\begin{equation}
    \mathcal{H}_i^* = \arg \min_{c, \Sigma, \mu, \alpha} \mathcal{L}_{rgb}(\mathcal{R} (\mathcal{H}_i), E_i)+ \arg \min_{m} \mathcal{L}_{KEA}(\mathcal{R} (\mathcal{H}_i), M_i),
    \label{eq:5}
\end{equation}
where $\mathcal{R}$ signifies the 3DGS rendering function.



% \indent \textbf{\textit{Photometric Loss.}}This initialization step involves learning a set of 3D Gaussians $\mathcal{H}_i$ to minimize the photometric discrepancy between the rendered and current frames $E_i$,
 We use the photometric loss $\mathcal{L}_{rgb}$ introduced in~\cite{kerbl20233d} which is a blend of $\mathcal{L}_1$ and D-SSIM losses:
\begin{equation}
    \mathcal{L}_{rgb} = (1-\gamma) \mathcal{L}_1 + \gamma \mathcal{L}_{\text{D-SSIM}},
\end{equation}
 

% However, the learning of parameter, $m$ is achieved through the KEA loss introduced below.

Given that our framework does not employ a pre-trained model on original (unedited) images, it is not feasible to un-project the posed 2D KEA identity labels onto the Gaussians using inverse rendering. Therefore, we learn the KEA identity of each Gaussian point during training by applying $\mathcal{L}_{KEA}$ loss ($\mathcal{L}_{KEA}$).

% \noindent\textbf{\textit{KEA Loss ($\mathcal{L}_{KEA}$).}}
$\mathcal{L}_{KEA}$ has two components to it. \textit{(i)} 2D Binary Cross-Entropy Loss, and  \textit{(ii)} 3D Jensen-Shannon Divergence (JSD) Loss, and is defined as,

\begin{equation}
    \mathcal{L}_{KEA} = \lambda_{BCE}\mathcal{L}_{BCE}+\lambda_{JSD}\mathcal{L}_{JSD}
\end{equation}

Let $N$ be the total number of pixels in the image, and $\mathcal{X}$ represent the set of all pixels. We calculate binary cross-entropy loss $\mathcal{L}_{BCE}$ as following, 

\begin{equation}
\begin{aligned}
\mathcal{L}_{BCE} = & -\frac{1}{N} \sum_{x \in \mathcal{X}} \bigg[ M_i(x) \log\left(\mathcal{R} (\mathcal{H}_i, m)(x)\right) \\
& + (1 - M_i(x)) \log\left(1 - \mathcal{R} (\mathcal{H}_i, m)(x)\right) \bigg]
\end{aligned}
\end{equation}
where $M(x)$ is the value of the ground truth mask at pixel $x$, indicating whether the pixel belongs to the foreground (1) or the background (0). The sum computes the total loss over all pixels, and the division by $N$ normalizes the loss, making it independent of the image size. A rendering operation, denoted as $\mathcal{R}(\mathcal{H}_i, m)(x)$ (see \textcolor{blue}{\textit{supply.}} for details), produces $m_{\mathcal{R}}$ for a given pixel $x$, which represents the weighted sum of the vector $m$ values for the overlapping Gaussians associated with that pixel. Here, $m$ and $m_{\mathcal{R}}$ both have a dimensionality of 2 which is intentionally kept the same as the number of classes in mask labels. We apply \textit{softmax} function on $m_{\mathcal{R}}$ to extract KEA identity given as,  $
 \text{KEA Identity} = \text{softmax}(m_{\mathcal{R}})$. The \textit{softmax} output is interpreted as either 0, indicating a position outside the KEA, or 1, denoting a location within the KEA.

To enhance the accuracy of Gaussian KEA identity assignment, we also introduce an unsupervised 3D Regularization Loss to directly influence the learning of Identity vector \(m\). This 3D Regularization Loss utilizes spatial consistency in 3D, ensuring that the Identity vector, $m$ of the top \(k\)-nearest 3D Gaussians are similar in feature space. Specifically, we employ a symmetrical and bounded loss based on the Jensen-Shannon Divergence,


\begin{equation}
\begin{aligned}
\mathcal{L}_{\text{JSD}} = & \frac{1}{2YZ} \sum_{y=1}^{Y}\sum_{z=1}^{Z} \Bigg[ S(m_y) \log\left(\frac{2S(m_y)}{S(m_y) + S(m'_z)}\right) \\
& +S(m'_z) \log\left(\frac{2S(m'_z)}{S(m_y) + S(m'_z)}\right) \Bigg]
\end{aligned}
\end{equation}
Here, $S$ indicates the \textit{softmax} function, and $m'_{z}$ represents the \textit{$z^{th}$} Identity vector from the $Z$ nearest neighbors in 3D space.



 
%  This can be mathematically represented as:
% $$
% \text{KEA Identity} = \text{softmax}(m_{\mathcal{R}})
% $$





% and assign KEA score, we unproject the posed 2D masks, $M$  back to the Gaussians with inverse rendering to update the parameter, $m$.
% It is worth mentioning that $\mathcal{L}_{rgb}$ doesn't update the parameter $m$ for the 3D Gaussians. 
% with $\lambda$ set to 0.2 for all experiments. This phase is notably efficient, requiring approximately 5 seconds to conform to the input frame $I_t$.

% \noindent\textbf{Pose Estimation through 3D Gaussian Transformation.}

\noindent\textbf{Relative Pose Initialization.} Next, the relative camera pose is estimated for each new frame added to the training scheme. ${\mathcal{H}_i}^*$ is transformed via a learnable SE-3 affine transformation $\mathcal{M}_i$ to the subsequent frame $i+1$, where $\mathcal{H}_{i+1}= \mathcal{M}_i  \odot \mathcal{H}_i$. Optimizing transformation $\mathcal{M}_i$ entails minimizing the photometric loss between the rendered image and the next frame $E_{i+1}$,
\begin{equation}
    {\mathcal{M}_i}^* = \arg \min_{\mathcal{M}_i} \mathcal{L}_{rgb}(\mathcal{R}(\mathcal{M}_i \odot\mathcal{H}_i), E_{i+1}\cdot M^{-1}_i ),
\end{equation}

% \begin{equation}
%     {\mathcal{M}_i}^* = \arg \min_{\mathcal{M}_i} \mathcal{L}_{rgb}\left(\begin{cases} 
%     \mathcal{R}(\mathcal{M}_i \odot \mathcal{H}_i), & \text{if } m_i = 0 \\
%     \text{Some other operation or value}, & \text{otherwise}
%     \end{cases}, E_{i+1}\cdot M^{-1}_i \right),
% \end{equation}



where, $M^{-1} = 1-M $, and the operation \(\mathcal{R}(\mathcal{M}_i \odot\mathcal{H}_i)\) is performed for 3D Gaussians with assigned KEA identity equal to 0 from the previous step. This decoupled optimization process is essential for learning $\mathcal{M}_i$ while functioning beyond the KEA, to circumvent challenges related to local minima that could emerge from even minor editing discrepancies.  In this optimization step, we keep the attributes of ${\mathcal{H}_i}^*$ fixed to distinguish camera motion from other Gaussian transformations such as pruning, densification, and self-rotation. 
Applying the above 3DGS initialization to sequential image pairs enables inferring relative poses across frames. However, accumulated pose errors could adversely affect the optimization of a global scene. To tackle this challenge, we propose the gradual, sequential expansion of the 3DGS.

% Represented as a quaternion $\mathbf{q}$ and a translation vector $\mathbf{t}$, the transformation $\mathcal{M}$ is optimized efficiently, typically within 5-10 seconds, given the proximity of adjacent frames.

% \subsection{Progressive Global 3DGS Development}\label{method:joint}
% Applying the above 3DGS initialization to sequential image pairs enables inferring relative poses across frames. However, accumulated pose errors could adversely affect the optimization of a global scene.

\noindent\textbf{3D Scene Expansion.}\label{method:joint} As illustrated above, beginning with frame $E_i$, we initiate with a collection of 3D Gaussian points, setting the camera pose to an orthogonal configuration. Then, we calculate the relative camera pose between frames $E_i$ and $E_{i+1}$. After estimating the relative camera poses, we propose to expand the 3DGS scene. This all-inclusive 3DGS optimization refines the collection of 3D Gaussian points, including all attributes, across $I$ iterations, taking the calculated relative pose and the two observed frames as inputs.  With the availability of the next frame $E_{i+2}$ after $I$ iterations, we repeat the above procedure: estimating the relative pose between $E_{i+1}$ and $E_{i+2}$, and expanding the scene with all-inclusive 3DGS.

To perform all-inclusive 3DGS optimization, we increase the density of the Gaussians currently under reconstruction as new frames are introduced. Following~\cite{kerbl20233d}, we identify candidates for densification by evaluating the average magnitude of position gradients in view-space. To focus densification on these yet-to-be-observed areas, we enhance the density of the universal 3DGS every $I$ step, synchronized with the rate of new frame addition. We continue to expand the 3D Gaussian points until the conclusion of the input sequence. Through the repetitive application of both frame-relative optimization and all-inclusive scene expansion, 3D Gaussians evolve from an initial partial point cloud to a complete point cloud that encapsulates the entire scene over the sequence. 

In our global optimization stage, we still utilize the $\mathcal{L}_{KEA}$ loss as new Gaussians are added during densification.
In addition to overcome the 2D editing incocnsistences, we propose pyramidal feature scoring where at the onset of training, we captures the attributes of all Gaussians and designates them as anchors. With each densification step, these anchors are updated to mirror the present attributes of the Gaussians. Throughout the training phase, an intra point cloud loss, $\mathcal{L}_{ipc}$ is utilized to compare the anchor state with the Gaussians' current state, maintaining that the Gaussians remain closely aligned with their initial anchors. Further, to optimise the estimated relative pose between subsequent Gaussian set, we introduce point cloud loss, $\mathcal{L}_{pc}$  similar as in~\cite{bian2023nope}. While we expand the scene, $\mathcal{L}_{ipc}$ limits the deviation of the Gaussian parameters while $\mathcal{L}_{pc}$ regularize the all-inclusive pose estimation.


\begin{equation}
\mathcal{L}_{\text{anchor}}^P = \sum_{i=0}^{n} \lambda_i (P_i - P_i^\prime)^2
\end{equation}
where $n$ is the total count of Gaussians and $P$ symbolizes a specific attribute of the Gaussian, chosen from the set $\{x, s, q, \alpha, c\}$. In this context, $P_i^\prime$ stands for the attribute's value in the anchor state. The coefficient $\lambda_i$ reflects the weight of the anchor loss for the $i$-th Gaussian, which is adjusted according to its inception phase.
The cumulative loss for training is articulated as:
\begin{equation}
\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{Edit}} + \sum_{P \in \{x, s, q, \alpha, c\}} \lambda_P \mathcal{L}_{\text{anchor}}^P
\end{equation}
Here, $\lambda_P$ denotes the weight of the anchor loss for attribute $P$, and $\mathcal{L}_{\text{Edit}}$ represents the editing loss as delineated in Sec.~\ref{pre: Editing Guidance}.

\begin{equation}
\mathcal{L}_{\text{anchor}}^P = \sum_{i=0}^{n} \lambda_i \sqrt{\sum_{j \in \mathcal{N}(i)} \min_{k \in \mathcal{N}^\prime(i)} \|P_j - P_k^\prime\|^2}
\end{equation}
where $n$ denotes the total number of Gaussians, and $P$ represents a specific attribute of the Gaussian, included in the set $\{x, s, q, \alpha, c\}$. Here, $P_j^\prime$ corresponds to the attribute's value in the anchor state for the nearest Gaussian $k$ to $j$, as determined by the Chamfer Distance. The set $\mathcal{N}(i)$ consists of points in the current state, while $\mathcal{N}^\prime(i)$ represents points in the anchor state. The parameter $\lambda_i$ indicates the weight of the anchor loss for the $i$-th Gaussian, adjustable based on its generation stage.
The overall training loss is then defined as:
\begin{equation}
\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{Edit}} + \sum_{P \in \{x, s, q, \alpha, c\}} \lambda_P \mathcal{L}_{\text{anchor}}^P
\end{equation}
In this equation, $\lambda_P$ signifies the strength of the anchor loss for attribute $P$, and $\mathcal{L}_{\text{Edit}}$ is the edit loss as specified in Sec.~\ref{pre: Editing Guidance}.



\begin{equation}
\mathcal{L}_{pc} =  CD (\mathcal{M}_i^*\mathcal{H}_i^*, \mathcal{H}_{i+1}^*)
% \arg \min_{\mathcal{M}_i} \mathcal{L}_{rgb}(\mathcal{R}(\mathcal{M}_i \odot\mathcal{H}_i), E_{i+1}\cdot M^{-1}_i ),
\end{equation}

where $CD$ is the chamfer distance. 
\begin{equation}
    \mathcal{L}_{T} = \lambda_{rgb}\mathcal{L}_{rgb}+\lambda_{KEA}\mathcal{L}_{KEA}+\lambda_{MSE\mathcal{L}_{MSE}+\lambda_{CD\mathcal{L}_{CD}
\end{equation}
This approach not only yields a photo-realistic reconstruction but also ensures precise camera pose estimation. For Global  



% \noindent \textbf{Multi-View Consistency Objective, $\mathit{L}_{\text{con}}$.}
% In this study, we aim to modify a single image to reconstruct an edited 3D scene. Given the constraints posed by view geometry in NeRF, ensuring spatial coherence presents a challenge. While cross-attention mechanisms facilitate editing within feature maps, it's imperative to define a loss function that fosters consistency across multiple views, thereby smoothing transitions in texture or color across adjacent views. Define the feature distribution for a 3D point $\bm{x}^j_p$ observed from $M$ source views as $\bm{e}^{j}_p = \{\bm{h}_1(\Pi_1(\bm{x}^j_p)), \ldots, \bm{h}_M(\Pi_M(\bm{x}^{j}_p))\}$, where $\bm{x}^j_p$ is sampled along ray $\bm{r}_j$. Consider another ray $\bm{r}_{j'}$, close or perturbed relative to $\bm{r}_j$. For each $\bm{x}^j_p$, we identify its nearest point $\bm{x}^{j'}_p$ on ray $j'$ by Euclidean distance, $d^{p}_{j,j'} = \|\bm{x}^j_p - \bm{x}^{j'}_p\|$. To enhance feature consistency at proximate points, we employ the Jensen-Shannon Divergence (JSD) loss,
% \begin{equation}
%     \mathit{L}_{J}(\bm{x}_p) = D_{\text{JSD}}(\bm{e}^{j}_p, \bm{e}^{j'}_p),
% \end{equation}
% where $\bm{e}^{j'}_p$ corresponds to the features from $\bm{r}_{j'}$. The symmetric property of JSD loss provides advantages over the Kullback–Leibler (KL) divergence~\cite{huszar2015not}, facilitating the rationale that closer points in pixel space should exhibit minimal feature space distances. We define the multi-view consistency loss with a weighted JSD loss as
% \begin{equation}
%     \mathit{L}_{\text{con}} = \sum_{p=1}^{P} \omega_p \mathit{L}_{\text{JSD}}(\bm{x}_p),
% \end{equation}
% where $\omega_p$ is the weight for the pair $(\bm{x}^j_p,\bm{x}^{j'}_p)$, calculated as $\omega_p = \frac{e^{-d^{p}_{j,j'}}}{\sum_{p=1}^{P} e^{-d^{p}_{j,j'}}}$. This formulation of $\mathit{L}_{\text{con}}$ enforces consistency across 3D points from different viewpoints, inherently encouraging geometric smoothness in the scene.


% \subsection{3D Scene Modification}
% \label{sec:3DSceneModification}

% \textbf{Removing Objects.} Direct elimination of Gaussians based on a mask might introduce visual discrepancies, particularly where the removed object meets other Gaussians. To mitigate this, we apply 2D inpainting methods to guide the reconstruction of these regions. Precise masks are essential for successful 2D inpainting. Post-deletion, we employ the K-nearest neighbors (KNN) algorithm to pinpoint Gaussians adjacent to the removed ones, typically at the boundary. These are projected onto different views, followed by mask dilation and hole correction to accurately delineate the boundary area, producing an enhanced mask for edge regions. This object removal process is usually completed within two minutes.

% \noindent\textbf{Adding Objects.} We outline this procedure as the introduction of new elements into the 3D Gaussian framework ${\theta}$, given a camera perspective $p$ and its corresponding view $I$, with the user specifying an inpainting region through a 2D mask $M$ on $I$. A textual prompt $y$ details the inpainting content. The goal is to update ${\theta}$ to accommodate the inpainting request.

% With $I$, $M$, and $y$, we first generate an inpainted 2D image $I^{M}_{y}$ using a 2D inpainting diffusion model, as described in \cite{podell2023sdxl}. The foreground object in $I^{M}_{y}$, as segmented by \cite{podell2023sdxl}, is then processed through an image-to-3D conversion method from \cite{long2023wonder3d} to create a preliminary 3D mesh. This mesh is converted into 3D Gaussians ${\theta}_y$, further refined as per the hierarchical Gaussian smoothing technique outlined in Sec.~\ref{sec: Hierarchical gs}.

% To integrate ${\theta}_y$ into the existing 3D structure ${\theta}$, we initially estimate the depth of $I^{M}_{y}$ using the method from \cite{ranftl2021vision}, aligning it with the depth map produced by ${\theta}$ at the same camera position through a least squares approach. This step ensures the precise placement and scaling of the newly inpainted object within ${\theta}$'s coordinate framework. After adjusting ${\theta}_y$ to fit within ${\theta}$, the two are merged, finalizing the updated 3D scene.

% Remarkably, this entire process of object addition is efficiently designed to take about five minutes.


% \subsection{Hierarchical Gaussian Splatting}
% \label{sec:hierarchical_gaussian_splatting}

% The foundational strength of conventional GS~\cite{kerbl3Dgaussians} in reconstruction tasks is attributed to the superior initialization facilitated by SFM-derived point clouds~\cite{schonberger2016structure}, in conjunction with consistent supervision from authentic datasets.

% The dynamics shift within generative contexts. Prior engagements with GS in text-to-3D and image-to-3D transitions~\cite{tang2023dreamgaussian,chen2023text,yi2023gaussiandreamer} have revealed GS's vulnerabilities to the unpredictability of generative guidance, owing to its resemblance to a point cloud-like representation. This instability stems from GS's direct susceptibility to the erratic nature of loss functions, contrasting with the implicit memorization and moderation capabilities inherent in neural network-based implicit representations. The routine updates involving a substantial quantity of Gaussian points per training step deprive GS of the detailed outcomes achievable through neural network-based implicit representations due to GS's excessive volatility, which impedes its convergence in generative training.



% To mitigate these issues, we propose Hierarchical Gaussian Splatting (HGS), a structured GS representation more amenable to generative and editing scenarios. HGS organizes GS into distinct generations according to the densification phase of their genesis. Initial Gaussians ${\Theta}$ receive a generational classification of $0$. As the editing training progresses, points engendered during the $k$-th densification phase are designated as generation $k$.

% This structured approach enables the application of variable constraints on Gaussians across different generations, modulating their adaptability. With the maturation of generations, the imposed constraints intensify. An anchor loss is employed to enforce these constraints, with HGS documenting the attributes of all Gaussians as anchors at training's












 % applying gradient back-propagation exclusively within $\mathcal{H}_{\text{KEA}}$. This ensures that only the designated RoI areas receive gradients during back-propagation. Optimization follows, utilizing these gradients to refine the scene. Through iterative optimization rounds, we achieve the final optimized scene representation $\mathcal{H}$.






==> sec/backup/related_work.tex <==
\begin{figure}[t!]
\vspace{-5mm}
\centering
    \includegraphics[width=1\linewidth, trim={1cm 3cm 1cm 3cm}, clip]{figures/figure3.pdf}
\vspace{-2mm}
\caption{\footnotesize {Comaprsion of method umar}}
\label{fig:fig3}
\end{figure}

\section{Related Work}
\label{sec:related_work}

\noindent\textbf{2D Image Editing via Diffusion Models} Recent breakthroughs in diffusion model technology~\cite{ho2020denoising, sohl2015deep} have enabled the generation of highly realistic images through advanced generative models~\cite{saharia2022photorealistic}. These models have demonstrated exceptional capabilities in creating detailed images from textual descriptions~\cite{dhariwal2021diffusion, ho2022cascaded, saharia2022palette, saharia2022image, song2019generative}, leveraging their profound understanding of semantics and powerful image generation potential. A growing body of research is exploring diffusion models for text-driven image editing, introducing techniques that allow for precise modifications based on user-provided instructions~\cite{nichol2021glide, ramesh2022hierarchical, rombach2022high, saharia2022photorealistic}. While some approaches require explicit before-and-after captions~\cite{hertz2022prompt} or specialized training~\cite{ruiz2023dreambooth}, making them less accessible to non-experts, iP2P~\cite{brooks2022instructpix2pix} simplifies the process by enabling direct textual edits on images, making advanced editing tools more widely accessible.

\begin{figure}[t!]
\vspace{-5mm}
\centering
    \includegraphics[width=1\linewidth, trim={1cm 3cm 1cm 3cm}, clip]{figures/figure3.pdf}
\vspace{-2mm}
\caption{\footnotesize \textbf{Teaser (Add bulldozer and object removal results@azib)}}
\label{fig:fig4}
\end{figure}




% \begin{figure}[t!]
% \vspace{-5mm}
% \centering
%     \includegraphics[width=1\linewidth, trim={1cm 1.5cm 1cm 1cm}, clip]{figures/figure2.pdf}
% \vspace{-2mm}
% \caption{\footnotesize \textbf{Figure2: kkkkkkkkkkk}}
% \label{fig:comparison}
% \end{figure}

\noindent\textbf{3D Scene Editing} The field of 3D Scene Editing of Radiance Fields is burgeoning, with a focus on altering the geometry and appearance of 3D scenes~\cite{liu2021editing, michel2022text2mesh, hong2022avatarclip, wang2022clip, kobayashi2022decomposing, tschernezki2022neural, bao2023sine, gao2023textdeformer, noguchi2021neural, liu2022nerf, li2022climatenerf, xu2022deforming, yang2022neumesh, xu2023instructp2p, li2023focaldreamer}. Traditional NeRF representations, however, pose significant challenges for precise editing due to their implicit nature, leading to difficulties in localizing edits within a scene. Earlier efforts have mainly achieved global transformations~\cite{nerfart, chiang2022stylizing, huang2021learning, huang2022stylizednerf, nguyen2022snerf, zhang2022arf, wu2022palettenerf}, with object-centric editing remaining a challenge. IN2N~\cite{haque2023instruct} introduced user-friendly text-based editing, though it might affect the entire scene. Attempts to localize edits through relevance mapping~\cite{mirzaei2023watchyoursteps} have been hindered by the limitations of 2D models like IP2P~\cite{brooks2022instructpix2pix}. The advent of 3D Gaussians~\cite{kerbl20233d} offers a promising solution with its explicit representation, enabling precise control over the editing regions, further enhanced by the integration of Large Language Models (LLMs) for a more automated editing process. Nevertheless, existing 3D editing models universally necessitate Structure-from-Motion (SfM) preprocessing. Recent studies like Nope-NeRF~\cite{bian2023nope}, BARF~\cite{lin2021barf}, and SC-NeRF~\cite{jeong2021self} have introduced methodologies for pose optimization and calibration concurrent with the training of \textit{(unedited)} NeRF. However, in this study, we explore a unique approach to constructing a 3D scene directly from a textual prompt, integrating frames from a monocular video without relying on any initial poses which brings unique challenges. We focus on utilizing the superior capabilities of Gaussian Splatting's explicit representation, enabling us to edit 3D models effectively by applying a pre-trained 2D editing diffusion model.

% \noindent\textbf{Pose-Free 3D Scene Construction.} The pursuit of bypassing the traditional Structure-from-Motion (SfM) preprocessing in Neural Radiance Fields (NeRFs) has garnered increasing attention in recent research. Initial endeavors, such as i-NeRF~\cite{yen2021inerf}, took steps toward this goal by predicting camera poses through keypoint matching with a pre-trained NeRF model. More recently, approaches integrating pre-trained networks for monocular depth or optical flow estimation have emerged, providing geometric or correspondence priors. For instance, Nope-NeRF~\cite{bian2023nope} incorporates depth priors derived from monocular depth estimation to enhance training fidelity. Furthermore, methods like VideoAE~\cite{Lai21a}, RUST~\cite{sajjadi2023rust}, MonoNeRF~\cite{fu2023mononerf}, and FlowCam~\cite{smith2023flowcam} aim to derive a generalizable scene representation from videos without predefined poses, although their performance in view synthesis often falls short without scene-specific optimization.

In this study, we explore a unique approach to constructing a 3D scene directly from a textual prompt, integrating frames from a monocular video without relying on any initial poses. We focus on utilizing the superior capabilities of Gaussian Splatting's explicit representation, enabling us to edit 3D models effectively by applying a pre-trained 2D editing diffusion model.

% Subsequent developments, including NeRFmm~\cite{wang2021nerfmm}, have explored the simultaneous optimization of NeRF networks alongside camera pose embeddings to refine this process. Despite improvements with SiNeRF~\cite{xia2022sinerf}, which utilizes SIREN-MLP~\cite{sitzmann2020implicit} and a novel sampling strategy, the focus remains predominantly on scenes with limited orientation changes. Efforts like BARF~\cite{lin2021barf} and GARF~\cite{chng2022garf} address the challenges posed by positional embedding's high-frequency components, with strategies such as coarse-to-fine optimization of camera poses alongside NeRFs, though still necessitating accurate initial camera pose approximations. 

